MARS: Processing-In-Memory Acceleration of Raw Signal Genome Analysis Inside the Storage Subsystem

Raw signal genome analysis (RSGA) has emerged as a promising approach to enable real-time genome analysis by directly analyzing raw electrical signals. However, rapid advancements in sequencing technologies make it increasingly difficult for software-based RSGA to match the throughput of raw signal generation. This paper demonstrates that while hardware acceleration techniques can significantly accelerate RSGA, the high volume of genomic data shifts the performance and energy bottleneck from computation to I/O data movement. As sequencing throughput increases, I/O overhead becomes the main contributor to both runtime and energy consumption. Therefore, there is a need to design a high-performance, energy-efficient system for RSGA that can both alleviate the data movement bottleneck and provide large acceleration capabilities. We propose MARS, a storage-centric system that leverages the heterogeneous resources within modern storage systems (e.g., storage-internal DRAM, storage controller, flash chips) alongside their large storage capacity to tackle both data movement and computational overheads of RSGA in an area-efficient and low-cost manner. MARS accelerates RSGA through a novel hardware/software co-design approach. First, MARS modifies the RSGA pipeline via two filtering mechanisms and a quantization scheme, reducing hardware demands and optimizing for in-storage execution. Second, MARS accelerates the RSGA steps directly within the storage by leveraging both Processing-Near-Memory and Processing-Using-Memory paradigms. Third, MARS orchestrates the execution of all steps to fully exploit in-storage parallelism and minimize data movement. Our evaluation shows that MARS outperforms basecalling-based software and hardware-accelerated state-of-the-art read mapping pipelines by 93x and 40x, on average across different datasets, while reducing their energy consumption by 427x and 72x.

==> acronyms.tex <==
\newacronym{ADI}{ADI}{Alternating Direction Implicit}
\newacronym{AGU}{AGU}{Address Generation Unit}
\newacronym[longplural={Access History Tables}]{AHT}{AHT}{Access History Table}
\newacronym{AHT-R}{AHT-R}{Access History Table - Read}
\newacronym{AHT-W}{AHT-W}{Access History Table - Write-Back}
\newacronym{AIP}{AIP}{Access Interval Predictor}
\newacronym{AL}{AL}{Added Latency for column accesses}
\newacronym{ASIC}{ASIC}{Application Specific Integrated Circuit}
\newacronym{AVX}{AVX}{Advanced Vector Extensions}
\newacronym[longplural={Basic Block Vectors}]{BBV}{BBV}{Basic Block Vector}
\newacronym{BHT}{BHT}{Branch History Table}
\newacronym{HBM}{HBM}{Hybrid Bandwidth Memory}
\newacronym{DDR4}{DDR4}{Double-Data Rate 4}
\newacronym{MIMD}{MIMD}{multiple-instruction multiple-data}
\newacronym{SIMT}{SIMT}{Single Instruction Multiple Threads}
\newacronym{SLP}{SALP}{subarray-level parallelism}
\newacronym{BLP}{BLP}{bank-level parallelism}

\newacronym{NN}{NN}{neural network}
\newacronym{BTB}{BTB}{Branch Target Buffer}
\newacronym{CAS}{CAS}{Column Address Strobe}
\newacronym{AMAT}{AMAT}{Average Memory Access Time}
\newacronym{CCD}{CCD}{Column to Column Delay}
\newacronym{AI}{AI}{Arithmetic Intensity}
\newacronym[longplural={Columnar Database Systems}]{CDBS}{CDBS}{Columnar Database System}
\newacronym[longplural={Chip Multiprocessors}]{CMP}{CMP}{Chip Multiprocessor}
\newacronym{CMT}{CMT}{Chip Multithreading}
\newacronym[longplural={Coarse-Grain Reconfigurable Arrays}]{CGRA}{CGRA}{Coarse-Grain Reconfigurable Array}
\newacronym{C-RAM}{C-RAM}{Computational-RAM}
\newacronym{CWD}{CWD}{Column Write Delay}
\newacronym{DBI}{DBI}{Dynamic Binary Instrumentation}
\newacronym[longplural={Database Management Systems}]{DBMS}{DBMS}{Database Management System}
\newacronym{DDR}{DDR}{Double Data Rate}
\newacronym{DEWP}{DEWP}{Dead Line and Early Write-Back Predictor}
\newacronym{DRAM}{DRAM}{Dynamic Random Access Memory}
\newacronym{DSBP}{DSBP}{Dead Sub-Block Predictor}
\newacronym{DSM}{DSM}{Decomposed Storage Manage}
\newacronym{FAW}{FAW}{Four row Activation Window}
\newacronym{FP}{FP}{Floating-Point}
\newacronym{EDP}{EDP}{Energy-Delay Product}
\newacronym{FCFS}{FCFS}{First-Come First-Serve}
\newacronym{FIFO}{FIFO}{Fist In, First Out}
\newacronym{FSM}{FSM}{finite state machine}
\newacronym{FPGA}{FPGA}{Field-Programmable Gate Array}
\newacronym[longplural={Functional Units}]{FU}{FU}{Functional Unit}
\newacronym{GAg}{GAg}{Global Adaptive branch prediction using one Global PHT}
\newacronym{GAs}{GAs}{Global Adaptive branch prediction using per-Set PHT}
\newacronym{GCC}{GCC}{GNU Compiler Collection}
\newacronym{GEMS}{GEMS}{General Execution-driven Multiprocessor Simulator}
\newacronym[longplural={General Purpose Processors}]{GPP}{GPP}{General Purpose Processor}
\newacronym{HMC}{HMC}{Hybrid Memory Cube}
\newacronym{HIVE}{HIVE}{HMC Instruction Vector Extensions}
\newacronym{IATAC}{IATAC}{Inter-Access Time per Access Count}
\newacronym{ILP}{ILP}{Instruction Level Parallelism}
\newacronym{IPC}{IPC}{Instructions per Cycle}
\newacronym{ISA}{ISA}{Instruction Set Architecture}
\newacronym{IRAM}{IRAM}{Intelligent RAM}
\newacronym{KIPS}{KIPS}{Kilo Instructions per Second}
\newacronym{LDS}{LDS}{Linked Data Structure}
\newacronym{LFSR}{LFSR}{Linear Feedback Shift Register}
\newacronym{LFMR}{LFMR}{Last-to-First Miss-Ratio}
\newacronym{MLP}{MLP}{Memory-Level Parallelism}

\newacronym{LLC}{LLC}{last-level cache}
\newacronym{LRU}{LRU}{Least Recently Used}
\newacronym{LSU}{LSU}{Load Store Unit}
\newacronym{LTP}{LTP}{Last-Touch Predictor}
\newacronym{LvP}{LvP}{Live-time Predictor}
\newacronym{LWP}{LWP}{Last Write Predictor}
\newacronym{MARSS}{MARSS}{Micro Architectural and System Simulator}
\newacronym{McPAT}{McPAT}{Multi-core Power, Area, and Timing}
\newacronym{MIPS}{MIPS}{Microprocessor without Interlocked Pipeline Stages}
\newacronym{MOB}{MOB}{Memory Order Buffer}
\newacronym{MMU}{MMU}{memory management unit}
\newacronym{PuD}{PUD}{processing-using-DRAM}
\newacronym{MPKI}{MPKI}{Misses per Kilo-Instruction}
\newacronym{MSHR}{MSHR}{Miss-Status Handling Registers}
\newacronym{NAS}{NAS}{Numerical Aerodynamic Simulation}
\newacronym{NDP}{NDP}{Near-Data Processing}
\newacronym{NMP}{NMP}{Near Memory Processor}
\newacronym{NoC}{NoC}{Network-on-Chip}
\newacronym{NPB}{NPB}{NAS Parallel Benchmark}
\newacronym{NUCA}{NUCA}{Non-Uniform Cache Architecture}
\newacronym{NUMA}{NUMA}{Non-Uniform Memory Access}
\newacronym{OoO}{OoO}{Out-of-Order}
\newacronym{OpenMP}{OpenMP}{Open Multi-Processing}
\newacronym{OS}{OS}{Operating System}
\newacronym{PAg}{PAg}{Per-address Adaptive branch prediction using one Global PHT}
\newacronym{PAs}{PAs}{Per-address Adaptive branch prediction using per-Set PHT}
\newacronym{PC}{PC}{Program Counter}
\newacronym[longplural={Pointer-Chasing Engines}]{PCE}{PCE}{Pointer-Chasing Engine}
\newacronym{PCM}{PCM}{Performance Counter Monitor}
\newacronym{PIM}{PIM}{processing-in-memory}
\newacronym[longplural={Pattern History Tables}]{PHT}{PHT}{Pattern History Table}
\newacronym{RAPL}{RAPL}{Running Average Power Limit}
\newacronym{GEMM}{GEMM}{general matrix-matrix multiplication}
\newacronym{RAS}{RAS}{Row Address Strobe}
\newacronym{RAT}{RAT}{Registers Alias Table}
\newacronym{RC}{RC}{Row Cycle}
\newacronym{RCD}{RCD}{RAS to CAS Delay}
\newacronym[longplural={Row-based Database Systems}]{RDBS}{RDBS}{Row-based Database System}
\newacronym{ROB}{ROB}{Reorder Buffer}
\newacronym{RRD}{RRD}{Row to Row activation Delay}
\newacronym{DNN}{DNN}{Deep Neural Network}
\newacronym{ANN}{ANN}{Artificial Neural Network}
\newacronym{PnM}{PNM}{processing-near-memory}
\newacronym{PuM}{PUM}{processing-using-memory}
\newacronym{FFD}{FFD}{first-fit-decreasing}
\newacronym{HFF}{HFF}{helper flip-flop}
\newacronym{OBPS}{OBPS}{one-bit per-subarray}
\newacronym{ABOS}{ABOS}{all-bits in one-subarray}
\newacronym{ABPS}{ABPS}{all-bits per-subarray}
\newacronym{GEMV}{GEMV}{general matrix-vector product}


\newacronym{RBR}{RBR}{redundant binary representation}
\newacronym{RP}{RP}{Row Precharge}
\newacronym{RTL}{RTL}{Register Transfer Level}
\newacronym{RTP}{RTP}{Read To Precharge}
\newacronym{RVU}{RVU}{Reconfigurable Vector Unit}
\newacronym{SDP}{SDP}{Skewed Dead-Block Predictor}
\newacronym{SESC}{SESC}{Superescalar Simulator}
\newacronym{SSE}{SSE}{Streaming SIMD Extensions}
\newacronym{SFP}{SFP}{Spatial Footprint Predictor}
\newacronym{SiNUCA}{SiNUCA}{Simulator of Non-Uniform Cache Architectures}
\newacronym{SMT}{SMT}{Simultaneous Multi-Threading}
\newacronym{SIMD}{SIMD}{single-instruction multiple-data}
\newacronym{LUT}{LUT}{Lookup Table}

\newacronym{SPEC}{SPEC}{Standard Performance Evaluation Corporation}
\newacronym{SoC}{SoC}{System-on-Chip}
\newacronym{SPP}{SPP}{Spatial Pattern Predictor}
\newacronym{SRAM}{SRAM}{Static Random Access Memory}
\newacronym{SSOR}{SSOR}{Symmetric Successive Over-Relaxation}
\newacronym{SSV}{SSV}{Search Set Vector}
\newacronym{TLB}{TLB}{Translation Look-aside Buffer}
\newacronym{TLP}{TLP}{Thread Level Parallelism}
\newacronym[longplural={Through-Silicon Vias}]{TSV}{TSV}{Through-Silicon Via}
\newacronym{VWQ}{VWQ}{Virtual Write Queue}
\newacronym{WTR}{WTR}{Write Recovery time}
\newacronym{WR}{WR}{Write To Read delay time}
\newacronym{TRA}{TRA}{triple row activation}


==> sections/11acknowledgements.tex <==
\section*{Acknowledgments}

\noindent We thank the anonymous reviewers of ICS 2025, \revB{ISCA 2025 and HPCA 2025} for their feedback. We thank the SAFARI group members for the feedback and stimulating intellectual environment they provide. We
acknowledge the generous gifts from our industrial partners including Google, Huawei, Intel, and Microsoft. 
This work is supported in part by the ETH Future Computing Laboratory
(EFCL), Huawei ZRC Storage Team, Semiconductor Research
Corporation, AI Chip Center for Emerging Smart Systems
(ACCESS), sponsored by InnoHK funding, Hong Kong SAR,
and European Union’s Horizon programme for research and
innovation [101047160 - BioPIM].

==> sections/9discussion.tex <==
\section{Discussion}
To our knowledge, \proposal is the \textit{first} work that combines different modes of computation within the storage system to reduce both data movement and computational overheads of an application. 
%Our approach leverages the unique features of the storage system (i.e., heterogeneous resources and large and dense capacity) to provide an efficient solution. 
%We believe that \proposal has a broad applicability beyond read mapping purposes. 
Currently, \proposal supports only read mapping  that does not require the end-to-end alignment performed by dynamic programming algorithms such as DTW~\cite{muller2007dynamic}.
However it can also be leveraged as a mechanism that quickly identifies seed hits used in full-alignment pipelines.
In this context, MARS accelerators can be repurposed and operate in synergy with the DTW part of such workflows.
Moreover, the compute primitives (i.e., arithmetic operations, filtering, sorting) implemented in our design, are applicable to both basecalled and raw signal genome analysis as well as other I/O intensive algorithms with similar data- and compute-intensive requirements (e.g., ML, NLP, image processing, and graph-based applications).
%These algorithms could be enabled on our hardware by adjusting our control FSM in the SSD controller.
%Additionally, the design allows for software tuning of key input parameters (e.g., window size, filter thresholds, input data type), enabling analysis of different genome sizes and optimization for various design parameters.
We hope that these insights can lead to solutions to similar overheads in other applications and inspire a a storage-centric accelerator and architecture design approach for data- and I/O-intensive applications.
% \begin{itemize}
%     \item The proposed \proposal architecture introduces a novel approach to RSGA by integrating multiple data-centric compute paradigms within an SSD to significantly enhance performance, energy efficiency, and scalability. This work represents a first-of-its-kind orchestration of PUM and PNM techniques within an SSD, optimized for genome analysis.
%     \item While the design builds on previous microarchitectural techniques, \proposal uniquely combines these methods within an SSD framework. This integration facilitates optimized data and control flow, improving latency and energy consumption significantly.
%     \item The architectural design is flexible enough to accommodate various algorithms based on the same compute primitives, such as arithmetic operations, filtering, and sorting, with slight modifications to the control flow.
%     \item \proposal demonstrates its application to an end-to-end genome analysis pipeline, achieving substantial improvements in latency and energy efficiency. This is achieved through algorithmic enhancements and efficient orchestration of compute resources within the SSD.
%     \item Suitable for related bioinformatics applications requiring large-scale data sorting, filtering, and dynamic programming. Adaptable for other computational fields needing efficient large-scle data processing (e.g., big data analytics, machine learning, real-time signal processing), either with adaptions to control unit only or by augmenting the system with additional dedicated compute units
%     \item We hope to inspire rethinking accelerator and architecture design for data- and I/O-intensive applications by using a storage-centric design principle to minimize time spend on data movement.
% \end{itemize}



==> sections/old-intro.tex <==
\section{Introduction}
\label{sec:Intro}


Identifying and analyzing the DNA sequence of an organism's genome, mainly referred to as \emph{genome analysis}, enable important advances in areas such as personalized medicine~\cite{alkan2009personalized,ashley_precision_2016,flores_p4medicine_2013, sweeney_rapid_2021}, outbreak tracing~\cite{Bloom_nextgen_2021,yelagandula_multiplexed_2021}, and evolutionary biology~\cite{romiguier_comparative_2014,ellegren_determinants_2016,Prado-Martinez_greatape_2013}. Genome analysis has two main steps: (1)~The generation of the genomic data, called \emph{genome sequencing} and (2)~a computational pipeline to analyze the genomic data \cite{firtina_rawhash_2023,zhang_sigmap_2021,kovaka_uncalled_2021,Bao2021Squigglenet,bonito, bingol2021gatekeeper,li_minimap2_2018,Poplin2018universal,lindegger2023rawalign,Li_mapping_2008}. 
%enabling other downstream tasks on the pre-processed data \cite{Poplin2018universal,lindegger2023rawalign,Li_mapping_2008}.

Nanopore sequencing is a widely-used high-throughput genome sequencing technique that can sequence long fragments of nucleic acid molecules (i.e., DNA or RNA), called \emph{reads}, with up to a few million bases (i.e., DNA characters of A, T, G, C)~\cite{jain_nanopore_2018} at relatively low cost~\cite{shendure_dna_2017}.
%generate large amounts of genomic data at relatively low cost~\cite{shendure_dna_2017}.
%In genome sequencing, high-throughput sequencing (HTS) can generate large amounts of genomic data at relatively low cost~\cite{shendure_dna_2017}. Nanopore sequencing is one of the most widely-used HTS technologies that can sequence long fragments of nucleic acid molecules (i.e., DNA or RNA), called \emph{reads}, with up to a few million bases (i.e., DNA characters of A, T, G, and C)~\cite{jain_nanopore_2018}. 
In nanopore sequencing, electrical current changes are measured while the DNA fragment moves
%at a certain throughput 
through a tiny pore, called \emph{nanopore}. The electrical current measurements, referred to as \emph{raw signals}, are subsequently analyzed to identify the genetic composition of the DNA fragment~\cite{kovaka_uncalled_2021,zhang_sigmap_2021,firtina_rawhash_2023,firtina_rawhash2_2023,li_minimap_2016,li_minimap2_2018}.
Compared to other sequencing technologies, nanopore sequencing offers two unique benefits: It provides (1) portability enabled through a compact device~\cite{jain_minion_2016}, facilitating scalable analysis for applications such as outbreak tracing and remote disease diagnosis~\cite{Greninger2015rapid,Kafetzopoulou2018assesment}, and (2) efficient sequencing time reduction by stopping the sequencing early based on the results of the computational analysis~\cite{loose_real-time_2016,payne_readfish_2021}.
%thereby providing opportunities for many important applications that require scalable and quick analysis, such as outbreak tracing~\cite{Mongan2020portable,Bloom_nextgen_2021} and disease diagnosis in remote locations~\cite{Greninger2015rapid,Kafetzopoulou2018assesment}
%First, it enables portable, high-throughput sequencing through a compact, lightweight device~\cite{jain_minion_2016}, thereby providing opportunities for many important applications that require scalable and quick analysis, such as outbreak tracing~\cite{Mongan2020portable,Bloom_nextgen_2021} and disease diagnosis in remote locations~\cite{Greninger2015rapid,Kafetzopoulou2018assesment}. 
%Second, nanopore sequencing allows early stopping of sequencing based on the results of the computational analysis (i.e., the initial part of the sequencing data provides enough information for analysis) to reduce sequencing time and cost.
To utilize these benefits, it is essential for the computational analysis pipeline to keep up with the rapid advances in nanopore sequencing in terms of speed and cost~\cite{Wang_nanopore_2021}.

Read mapping, a fundamental step in computational genome analysis pipelines, identifies the genomic origin and variations of a read by comparing it to a known genome of a certain species, called \emph{reference genome}~\cite{alser_accelerating_2020,alser_technology_2020}. 
%A fundamental step in many computational pipelines, that analyze genomic data, is called read mapping. To identify the genomic origin and variations of a read, the read mapping step finds potential similarities between a read and a known genome of a certain species, called \emph{reference genome}~\cite{alser_accelerating_2020,alser_technology_2020}. 
To find similarities accurately, conventional approaches use basecalling to translate noisy raw signals to sequences of nucleobase characters before performing read mapping~\cite{bonito,huang_sacall_2020,singh_framework_2022}.
%To find these similarities accurately, conventional approaches use a translation process called basecalling to interpret the raw signals as sequences of nucleobase characters before performing read mapping.~\cite{bonito,huang_sacall_2020,singh_framework_2022}.
%Conventional approaches use a translation process called basecalling to interpret the raw signals as sequences of nucleobase characters before continuing with further downstream analysis~\cite{bonito,huang_sacall_2020,singh_framework_2022}. 
Basecalling is usually very compute- and energy-intensive as it uses complex deep learning models to account for the noise in the raw signals~\cite{dunn_squigglefilter_2021,mao_genpip_2022}.
%Basecalling is usually very compute- and energy-intensive as they use complex deep learning models~\cite{dunn_squigglefilter_2021,mao_genpip_2022} to account for the noise in the raw signals introduced by variations in the properties of the nanopores or the conditions in which the sequencing is performed.
In contrast, recent approaches~\cite{kovaka_uncalled_2021,zhang_sigmap_2021,firtina_rawhash_2023,firtina_rawhash2_2023,shih_haru_2023,dunn_squigglefilter_2021,Bao2021Squigglenet}, which we refer to as \rsga (\RSGA), directly use raw signals without translating them to bases, to achieve faster, more energy-efficient mechanisms while aiming for accurate analysis.
%In contrast, recent approaches use \rsga~\cite{kovaka_uncalled_2021,zhang_sigmap_2021,firtina_rawhash_2023,firtina_rawhash2_2023,shih_haru_2023,dunn_squigglefilter_2021,Bao2021Squigglenet}, which directly operates on the current measurements given by the raw signals aiming for accurate analysis using faster and more energy-efficient mechanisms~\cite{shih_haru_2023,wan_beyond_2022}. 

Although \RSGA approaches reduce the computational load on the genome analysis pipeline by skipping the resource-intensive basecalling step, we observe three key problems in our motivational study: (1)~high I/O data movement overhead, (2)~a need for large computational resources, and (3) different needs for different genome sizes which all lead to high energy consumption.
%(\S\ref{sec:motivation}): 
(1)~Since read mapping operates on large data sets of up to hundreds of gigabytes~\cite{mao_genpip_2022}, it is susceptible to high data movement latency and energy consumption. We observe an average runtime slowdown of 67.5\% and 89.9\% and an average increase in energy consumption of 2.10x and 1.41x when comparing the execution of \RSGA on a cost- and performance optimized SSD to a system setup exposed to \emph{no} I/O data movement overhead (\S\ref{sec:motivation-why-isp}).
(2)~During read mapping in \RSGA, we observe that the computational intensive dynamic programming step, which identifies the similarities between the reference genome and the sequenced data~\cite{Kalikar2022mm2fast}, accounts for 74\% to 97\% of the total execution time. The resulting demand for server-grade or cloud computing resources can compromise the portability of genome sequencing due to increased power usage and poor scalability, and, for cloud computing, potentially lead to higher latency (\S\ref{sec:motivation-why-accelerate}).
(3)~We observe that genome sizes impact data movement and computational challenges differently. Smaller genomes are primarily affected by data movement overhead, whereas larger genomes additionally encounter computational bottlenecks. We conclude that a \RSGA system must be adaptable to various genome sizes by providing a low-power, high-performing system for read mapping while minimizing the observed data movement and computational bottlenecks.
%We observe that different genome sizes exhibit varying degrees of data movement and computational bottlenecks. Smaller genomes are more affected by data movement, while large genomes are more prone to the computational bottleneck. A \RSGA system must be flexible enough to handle various genome sizes and reduce their energy consumption by mitigating data movement and minimizing computational overheads.
%(2)~The read mapping step in \RSGA exhibits a significant computational bottleneck while identifying the similarities between the reference genome and the sequenced data, accounting for 74\% to 97\% of the total execution time. This phase primarily involves two computational primitives: sorting and dynamic programming. Both exhibit suboptimal cache hierarchy utilization, particularly given the data sizes typically encountered in raw signal genome analysis (\S\ref{sec:motivation-why-accelerate}).
%(3)~We observe that \RSGA, especially for larger genomes (e.g., human genome), require substantial compute resources, e.g., a server-grade setup or access to cloud computing, to enable high parallelism for real-time analysis. Requiring such extensive computational resources, especially for a lightweight portable sequencer, can compromise the portability of genome sequencing due to increased power usage and poor scalability, and, for cloud computing, potentially higher latency (\S\ref{sec:motivation-why-accelerate}). 
%In the read mapping phase of \RSGA, identifying similarities between the reference genome and sequenced data is computationally intensive, consuming 74% to 97% of total execution time. This phase, involving sorting and dynamic programming, struggles with cache hierarchy inefficiency, particularly with the large data sizes in raw signal genome analysis. Additionally, \RSGA demands significant compute resources, especially for larger genomes like the human genome. This need for server-grade or cloud computing resources can hinder the portability of genome sequencing, due to increased power consumption, scalability issues, and potential latency in cloud computing.
%(2)~Second, we observe that read mapping applications can harness significant parallelism. Nonetheless, this necessitates substantial computational resources, e.g., a server-grade setup or access to cloud computing. Given that sequencing is accessible in a portable, lightweight format, relying on extensive computational servers could compromise its portability, as well as lead to data privacy concerns and restricted usage in remote areas when relying on cloud computing.

Although there have been significant efforts to improve read mapping~\cite{liu_fast_2016,liao_subread_2013,laguna2020seed,bingol2021gatekeeper,alser2020sneakysnake,kim2018grim,alser2019shouji,dunn_squigglefilter_2021,laguna2020seed,turakhia2018darwin,cali2020genasm,guo2019hardware},
%with algorithmic~\cite{liu_fast_2016,liao_subread_2013,laguna2020seed,bingol2021gatekeeper,alser2020sneakysnake,kim2018grim,alser2019shouji} and system optimizations~\cite{dunn_squigglefilter_2021,laguna2020seed,turakhia2018darwin,cali2020genasm,guo2019hardware}, 
prior works have not explored the \RSGA approach to design a system that is scalable to larger genomes due to their two main limitations. 
First, existing designs accelerating read mapping do not apply to raw signal data as they require specialized matching algorithms due to the inherently noisy nature of raw signals. 
%Nanopore sequencing can produce varying signal amplitudes for identical DNA sequences due to the unique properties of each nanopore and the conditions in which the sequencing is performed~\cite{david_nanocall_2017}. 
Second, while \RSGA reduces the computational load on the pipeline by avoiding resource-intensive basecalling, the challenge of high data movement overhead remains, as detailed in \S\ref{sec:motivation-why-isp}. No prior accelerator suitable to work on raw signal input data~\cite{shih_haru_2023,dunn_squigglefilter_2021} considers the end-to-end pipeline and its key bottleneck of data movement in their design such that it is applicable to larger genomes.

\isp (ISP) could fundamentally solve the data movement problem by drastically cutting the I/O overhead. ISP adds computing capabilities to the storage device reducing the data transfer between the storage and processing unit, thereby enhancing efficiency and speed.
We identify three main challenges for In-Storage-Processing of \RSGA: (1)~executing a diverse set of compute primitives in the read mapping pipeline, (2)~ensuring high parallelism in computational capabilities near storage to achieve speedups for a wide range of genome sizes, and (3)~minimizing the newly introduced area and cost overheads in storage.
%First, we need to execute a diverse set of compute primitives in the read mapping pipeline. Second, the computational capabilities provided near the storage must be capable of high parallelism to compete with a compute-centric setup. Finally, the compute capabilities near and in storage should introduce as minimal area and cost overhead as possible. 
%By additionally providing specialized compute units near storage that can exploit the application's high parallelism, we can provide high computational capacity in a lightweight manner.

Our \textbf{goal} is to design a compact, end-to-end \isp system to improve the performance and energy efficiency of the state-of-the-art \rsga algorithm~\cite{firtina_rawhash_2023,firtina_rawhash2_2023} that is scalable to larger genomes.
We focus on addressing the aforementioned key challenges of ISP, accelerating bottlenecks, and maintaining accuracy while minimizing the data movement overhead.

To this end, we propose \emph{\proposal} (\textbf{Raw} Signal \textbf{G}enome \textbf{A}nalysis \textbf{I}n- and \textbf{N}ear-\textbf{S}torage), 
%the first end-to-end Processing-in-Storage Accelerator for \RSGA.
%the first accelerator for \RSGA scalable to large genomes.
the first \isp design combining \pum with \pnm technologies \emph{within} a NAND flash-based Solid State Drive (SSD). Our proposal extends beyond the configuration of a conventional, modern SSD consisting of an SSD controller, an array of flash chips, and a DRAM in SSD for caching frequently requested data and maintaining metadata~\cite{gupta_dftl_2009}.
%to execute an end-to-end real-world application
%SSDs are one of the most used storage devices from cloud environments to mobile devices~\cite{dirik_isca_2009,do2013query,cai-errors-2018,cho2013active,kim2018autossd,eshghi2018ssd,micheloni2010inside,cai2013threshold,cai2015data,cai2017error,park2022flash,kim2020evanesco,tavakkol2018flin}. Their high performance, low power consumption, and shock resistance make them a suitable replacement for other storage mediums like hard disk drives (HDDs)~\cite{dirik_isca_2009, mielke2017reliability, kryder2009after}. 
\proposal is leveraging and augmenting the components in this environment of SSDs by using a hardware-algorithm co-design approach to execute an end-to-end application based on two \textbf{key ideas}: (1)~We orchestrate multiple \isp approaches to create a heterogeneous computing environment in SSD which supports all compute primitives involved in \RSGA with minimal data movement and customized compute resources. (2)~We improve and simplify the \RSGA algorithm to reduce unnecessary computations and enhance its compatibility with hardware.
We realize \proposal based on three \textbf{key mechanisms}:

\noindent \textbf {1.~Heterogeneous Acceleration } We leverage and augment the rich environment SSDs provide by selecting one of the following ISP methods for \RSGA acceleration.
(1)~\emph{'Processing-near-SSD'} (PNS) and ~\emph{'\pnm'} (\PNM) add dedicated logic close to the SSD controller or the DRAM in storage.
(2)~\emph{'\pum'} (\PUM) exploits the analog properties of the DRAM in SSD to perform in-memory computations with minimal data movement overhead.
Different ISP methods provide different performance, energy efficiency, and area overhead trade-offs, allowing us to exploit the advantages of each method and tailor them to the compute primitives involved.
%. We analyze the computations involved in the targeted application and identify a specific ISP approach to perform and accelerate each computation most efficiently. We group these ISP approaches into two categories:
%(1)~We introduce dedicated logic close to the SSD controller to perform sorting and use the DRAM in SSD to cache intermediate results. We call this approach \emph{'Processing-near-SSD' (PnS)} as it adds additional logic to the SSD. 
%(2)~Further, we add computational units and exploit the analog properties of the DRAM in SSD to perform logic and arithmetic operations and enable the bulk execution of a LUT operations in DRAM to query a hash table. Both strategies are collectively termed \emph{'Processing-in-Memory' (PiM)}, emphasizing minimal changes to the memory's inherent organization. We refer to PiM methods relying on the inherent analog properties of the DRAM as \emph{'Processing-using-Memory' (PuM)} and to PiM methods that add logic to the DRAM as \emph{'Processing-near-Memory' (PnM)}.
%In this manner, we can exploit the advantages of different ISP techniques and tailor them to the respective compute primitive: We leverage the benefits of analog PuM in SSD, which mostly provides higher speed-ups and energy efficiency but is limited to simpler operations. In contrast, PnS and PnM introduce greater overhead in terms of speed, energy, and area, but they can handle more complex computations. By combining these different data-centric ISP primitives, we are able to execute \RSGA end-to-end within an augmented SSD system efficiently.

\noindent \textbf {2.~Hardware Compatibility } We enhance hardware compatibility by introducing a combination of additional filters to minimize the computational demand in an early stage of the application.
%thereby excluding low-quality potential mappings between the sequenced data and the reference genome. 
We transition from floating-point operations to fixed-point and integer operations with minimal accuracy loss, achieving efficient data-centric processing.
%enhancing the efficiency of data-centric processing and hardware-based methods.

\noindent \textbf {3.~Minimizing Data Movement } We mitigate the data movement bottleneck by processing in-place, leveraging dedicated compute units and the internal DRAM's analog properties. Using the ISP paradigm effectively reduces the I/O overhead while allowing quick access to large amounts of data.
%We mitigate the data movement bottleneck by processing the data where it is stored. \proposal is built upon the ISP paradigm: We leverage dedicated compute units, as well as the analog properties of the DRAM inside the SSD, to perform computations close to where the data resides. By operating close to the SSD, \proposal effectively reduces the I/O overhead while at the same time being able to access large amounts of data quickly.


%To evaluate \proposal, we use a combination of synthesized Verilog models and findings based on state-of-the-art simulation tools widely used for DRAM and SSD research, CACTI7~\cite{CACTI7} and MQSim~\cite{tavakkol2018mqsim}. 
Our evaluation includes latency, energy consumption, and area overhead and assesses the performance impact of the storage system design.
%We demonstrate the advantages of our algorithmic enhancements as standalone improvements and show the benefits of our end-to-end system design.
Since there is no existing system for \RSGA that scales to large genomes, we provide two additional hardware-accelerated design points during our evaluation to show the trade-offs of \proposal.
Compared to the state-of-the-art software implementation on a server-class CPU, \proposal improves end-to-end performance on average by 14.9$\times$, and the energy consumption by 170.3$\times$ (more evaluation points in \S\ref{sec:eval}).
%Compared to the state-of-the-art software implementation on a server-class CPU and a hardware-accelerated system, our design \proposal improves the end-to-end performance on average (up to) by 14.9x (53.2x) and 3.2x (x), and improves the energy consumption by 170.35x (320.12x) and 10.9x (x) system respectively.

This work makes the following \textbf{key contributions}:
\vspace{-.2em}
\squishlist
    % \item We assess the I/O data movement overhead in terms of execution time and energy consumption for \rsga based on insights from real genomic datasets from various organisms. We investigate computational constraints and explore opportunities for enhanced parallelism and early filtering, reducing the computational load.
    \item We evaluate I/O data movement overhead in \rsga in terms of energy consumption and performance using real genomic datasets. We analyze computational constraints and explore opportunities to improve parallelism and reduce computational load.
    \item We propose \proposal, the first HW-Algorithm Co-Design for \rsga scalable to large genomes.
    \item To our knowledge, \proposal is the first architecture that leverages multiple different data-centric computing approaches within an SSD device: We combine \pim in SSD with Processing-near-SSD to efficiently enable a wide variety of compute primitives involved in end-to-end \rsga.
\squishend







==> sections/old2background_shortened.tex <==
\section{Background}
\label{sec:background}

\subsection{Raw Signal Genome Analysis}
\label{sec:BG-RSGA}
Nanopore sequencing can sequence long fragments of DNA~\cite{jain_minion_2016, jain_nanopore_2018}, called \emph{reads}, by measuring the electrical current changes while the DNA fragment traverses a tiny pore, called \emph{nanopore}.
%Longer fragments improve the quality of the analysis~\cite{jain_nanopore_2018}. 
The generated sequence data~\cite{cali_nanopore_2017}, referred to as \emph{raw signals}, are required for downstream analysis for read mapping and variant calling purposes.
In the conventional genome analysis approach, raw signals are first translated into sequences of nucleobase characters (i.e., A, C, G, T), i.e. basecalling process ~\cite{alser_technology_2020,alser2022molecules}, and then mapped to a reference genome to find similarities ~\cite{bonito,huang_sacall_2020,singh_framework_2022}.
\RSGA replaces this computationally expensive approach ~\cite{dunn_squigglefilter_2021,mao_genpip_2022} by eliminating the need for basecalling and operating directly on the raw signals for read mapping purposes~\cite{kovaka_uncalled_2021,zhang_sigmap_2021,firtina_rawhash_2023,firtina_rawhash2_2023}.

%, need to be subsequently analyzed to identify the genetic composition of the DNA fragment~\cite{kovaka_uncalled_2021,zhang_sigmap_2021,firtina_rawhash_2023,firtina_rawhash2_2023,li_minimap_2016,li_minimap2_2018}.
%\kon{Nanopore sequencing offers two unique benefits: (1) portable genome analysis in a compact device and (2) sequencing time and cost reduction through early termination mechanisms Read Until~\cite{loose_real-time_2016} and Run Until~\cite{payne_readfish_2021} for an individual read and the entire sequencing run respectively.}
% To exploit these benefits, \emph{real-time analysis}~\cite{Mutlu2023Accelerating,firtina_rawhash2_2023} is required to match the nanopore sequencing throughput.
%There are two main approaches for real-time analysis.
%\kon{First, the conventional and heavily optimized analysis pipeline~\cite{alser_technology_2020,alser2022molecules}, that consists of two steps: 
%(1) basecalling, which translates raw signals into sequences of nucleobase characters (i.e., A, C, G, T) and 
%(2) read mapping, which finds potential similarities between a read and a \emph{reference genome}~\cite{bonito,huang_sacall_2020,singh_framework_2022}.} 
%Basecalling approaches lead to highly accurate results but are computationally demanding due to their reliance on deep learning models~\cite{dunn_squigglefilter_2021,mao_genpip_2022}. 
%\kon{To alleviate this overhead, the second and most recent approach~\cite{kovaka_uncalled_2021,zhang_sigmap_2021,firtina_rawhash_2023,firtina_rawhash2_2023}, i.e., \rsga (\RSGA), aims to avoid compute-intensive basecalling by directly mapping the raw signals to the reference genome.}

\RSGA typically requires the execution of two main steps.
First, a preparatory offline step, known as \emph{indexing}, stores short subsequences from reference genomes in a suitable data structure (e.g., a hash table) for quick search and matching of subsequences.  
Second, the \emph{online} (e.g., real-time) \emph{mapping} step, identifies similarities between the sequenced raw signals and reference genome by utilizing this index.
A typical state-of-the-art mechanism for \RSGA performs the offline indexing and online mapping following the steps shown in Fig.~\ref{fig:rawhash-flow}, leveraging an efficient data structure such as hash-tables ~\cite{firtina_rawhash_2023}.
To compare sequences of characters from the reference genome and sequences of raw signal values from the input sample, both reference subsequences and raw signals are converted into a series of values corresponding to certain genomic subsequences, known as \emph{events}.
Both reference and raw-signal events incur a quantization scheme, that reduces the sequencing noise from the signals and enables accurate comparisons between them.
For the reference, event detection and quantization takes places offline before the indexing, whereas for the raw nanopore signals \minorfix{event detection happens} online (Fig.~\ref{fig:rawhash-flow},~(1)).
During online mapping, the quantized values of the raw signal events \minorfix{are used to} generate hash values and the \emph{seeding} step queries the hash table to identify matching hash values quickly  (Fig.~\ref{fig:rawhash-flow},~(2)).
Last, to identify the similar regions between the reference genome and a raw signal, the \RSGA tool identifies several matching hash values (i.e., anchors) within close proximity to each other by using a computationally costly dynamic programming approach, called \emph{chaining} (Fig.~\ref{fig:rawhash-flow},~(3)).

\begin{figure}[tbh]
  \centering
  \includegraphics[width=0.85\columnwidth]{figures/RawHash-Flow.pdf}
  \caption{Overview of workflow in a typical \RSGA tool that leverages hash-tables for efficient indexing.}
  \label{fig:rawhash-flow}
\end{figure}

\subsection{SSD Architecture}

NAND flash-based Solid State Drives (SSDs) are the prevalent storage medium due to their high performance, low power consumption, and shock resistance~\cite{dirik_isca_2009, mielke2017reliability, kryder2009after,do2013query,cai-errors-2018,cho2013active,kim2018autossd,eshghi2018ssd,micheloni2010inside,cai2013threshold,cai2015data,cai2017error,park2022flash,kim2020evanesco,tavakkol2018flin}.
Fig.~\ref{fig:ssd-arch} depicts the architecture of a typical modern SSD, which consists of three main components: (1)~an array of NAND flash chips connected via flash channels to (2)~the SSD controller, and (3)~the DRAM in SSD for caching \minorfix{metadata and} frequently-requested data~\cite{gupta_dftl_2009}. 
% We provide more details about components related to our work.

\begin{figure}[tbh]
  \centering
  \includegraphics[width=0.8\columnwidth]{figures/SSD-Architecture.pdf}
  \caption{Organizational overview of a modern SSD.}
  \label{fig:ssd-arch}
\end{figure}

\noindent\textbf{1. NAND Flash and Bandwidth.}
NAND flash arrays store data in 4–16 KiB pages and are connected to the SSD controller via channels. 
The internal bandwidth (BW) of a modern SSD between NAND flash chips and the SSD controller usually surpasses the BW between the host and the SSD. 
% Recent enterprise SSD controllers~\cite{anandcontroller_2020} support 6.55GB/s external and 19.2GB/s internal BW, distributed across 16 channels at 1.2 GB/s each.
To bridge the performance gap between main memory and storage systems, SSD manufacturers enhance external BW via advanced I/O interfaces.
% For instance, cutting-edge PCIe-Gen4 SSDs can reach up to 8 GB/s for sequential-read BW (e.g., 7 GB/s in Samsung PM1735~\cite{samsungPM1735_2020}).}


\noindent\textbf{2. SSD Controller.}
It consists of two primary components: 1) multiple cores running the SSD firmware, i.e., the \emph{flash translation layer (FTL)}, and 2) per-channel hardware \emph{flash controllers} that (i) manage I/O request transfer between the SSD controller and the flash chips and (ii) provide error-correcting codes (ECC) for the NAND flash chips~\cite{tavakkol2018mqsim,gupta_dftl_2009,zhou2015efficient,lim2010faster}. 
FTL maintains logical-to-physical (L2P) address mappings for read operations, handles communication with the host system, internal I/O scheduling and various SSD management tasks to abstract the unique characteristics of NAND flash memory from the host. 

\noindent\textbf{3. Internal DRAM.}
Modern SSDs employ low-power DRAM to store metadata crucial for SSD management  \minorfix{(e.g., L2P page mapping table)} and to cache frequently accessed pages~\cite{gupta_dftl_2009}. 
Typically, the DRAM takes up 0.1\% of the SSD's capacity (e.g., 4GB LPDDR4 DRAM for a 4TB SSD~\cite{samsung860pro_2018}). 
As shown in Fig.~\ref{fig:dram-arch}, DRAM is organized in a hierarchical structure. 
% At the highest level, a DRAM module comprises multiple chips, each containing several banks (e.g., 8-16), subdivided into multiple subarrays (e.g., 64-128). 
% A subarray (SA in Fig.~\ref{fig:dram-arch}) is a 2D array of cells organized into multiple rows (e.g., 512-1024) and columns (e.g., 2-8kB)~\cite{kim2018solar,lee2017design}. 
%To read data, we set the row address to copy the relevant row content into the local row buffer. 
%The chosen column is then routed to the local data line via column selection lines.

\begin{figure}[tbh]
  \centering
  \includegraphics[width=0.85\columnwidth]{figures/DRAM-Organization.pdf}
  \caption{Organizational overview of a DRAM module.}
  \label{fig:dram-arch}
\end{figure}



==> sections/rebuttal.tex <==
\clearpage
\thispagestyle{empty}
\twocolumn


  
\noindent We thank the reviewers for their meaningful and constructive feedback. We will take into account all comments to improve our work for potential next submissions. Here, we responded as best as we can to concerns and questions for unclear parts of our work. 


\noindent
\textbf{Q1.Clarify DRAM size and use and potential scalability issues with larger datasets.
}
Our current setup targets an SSD with 4GB internal DRAM (Table 1). As the genome size scales, the hash table index eventually exceeds the limit of SSD-internal DRAM resources. To overcome this challenge, MARS design adopts a batching strategy that splits the index into independent batches, thus supporting parallel access to independent regions of the reference genome and increasing scalability. This strategy indeed incurs a data movement overhead of repeatedly loading a different batch of the index. 
However, despite the overhead MARS still achieves superior performance to other approaches.
%However, the overall latency gains of in-storage accelerated RSGA compensates for the added overhead.



\noindent
\textbf{Reviewer A}

\noindent
\textbf{A1. The choice of $thresh\_freq$ and $thresh\_voting$ seem arbitrary and not well-explained.}
Our selection is based on a parameter sweep that locally optimizes the threshold values. Initially, we test a broad set of commonly used parameters on a smaller dataset. We focus on identifying those that provide high accuracy while efficiently filtering a large volume of data. Once promising parameters are identified, we carry out a more exhaustive search within the ranges that performed well on the smaller dataset. This empirical exploration is validated by an independent input dataset. 

\noindent
\textbf{A2. Determining 16b width for fixed precision.}
We performed an experimental analysis on a software level and evaluated the accuracy achieved for fixed point arithmetic using 64,32,16 and 8 bytes. The use of 16 bytes guarantees minimal accuracy loss compared to floating point and significant resource utilization savings.
%On the other hand, choosing 8 bytes inflicts a significant drop in accuracy.

\noindent
\textbf{A3.Advantages of choosing a bitonic sorter over other sorting mechanisms.
}The bitonic sorter was chosen thanks to the parallelism capabilities and suitability for hardware implementation of the design. Regarding parallelism: 1) the sorting process can be broken down into parallel stages, and 2) it is a highly scalable and efficient algorithm for large datasets. Regarding hardware suitability 3) it has a predictable pre-defined number of steps and 4) it can be implemented with simple hardware-friendly operations.

\noindent
\textbf{A4.Applicability of hardware components to other applications beyond genomics.
}Our design covers essential compute primitives (i.e., arithmetic operations, filtering, sorting) that can be applied to other I/O intensive algorithms with similar data- and compute-intensive requirements (e.g., ML, NLP, image processing, and graph-based applications). 
%We hope that our design can serve as a paradigm of fully harvesting storage capabilities to accelerate such applications. 

\noindent
\textbf{Reviewer B}

\noindent
\textbf{B1. The proposed approach is incremental.}
Implementing RSGA in storage is challenging due to its high memory demands, irregular memory access, and computationally intensive tasks. To overcome these issues, we propose the first ISP system that employs multiple different data-centric computing approaches within the SSD device. While some components are inspired by prior work, our key contribution lies in their systematic integration for efficient end-to-end execution, ensuring they complement rather than interfere with each other. Our design can serve as a paradigm of fully harvesting storage capabilities to accelerate similar applications.

\noindent
\textbf{B2. How does the added complexity contribute to the performance when compared to a single type of PIM approach? }
In Section 7.2, Fig.11, we evaluate the effectiveness and performance of our design  against two designs based on the PIM paradigm only: MS-EXT and GenPIP. MARS yields better results in terms of latency than these designs across all datasets. Similarly, MARS achieves better energy results than these designs, as shown in Fig. 12.

\noindent
\textbf{B3. Impact of fixed-point type conversion on performance and energy.
}
In Section 7.2, Fig.11 and Fig.12, we evaluate the impact of fixed-point type conversion on performance and energy respectively, by considering a software-only MARS pipeline that only adopts the fixed-point type conversion and comparing it against the floating point based pipeline.

\noindent
\textbf{Reviewer C}

\noindent
\textbf{C1. Clearly explain why one would adopt RSGA, compared to basecalling approach.}
\RSGA is a recent paradigm in bioinformatics pipelines and exhibits significant benefits such as: 1) it preserves richer information of raw signals for downstream analysis and leads to novel or more accurate analysis and 2) reduces the computational overhead of basecalling-based approaches. \RSGA approaches already deliver better performance than optimized basecalling pipelines,therefore it is a promising direction as a standalone or complementary stage.


\noindent
\textbf{C2. It is also unclear why in Fig 11 and 12, the GPU based BC technique trails CPU based RH technique.}
This performance enhancement is mainly attributed to the elimination of the basecalling step, despite it taking place on GPU, and highlights how promising RSGA is.

\noindent
\textbf{Reviewer D}

\noindent
\textbf{D1. Questions regarding RawHash, DTW and flexibility of MARS.}
First, we would like to clarify that this work builds upon the RawHash2 pipeline, not RawHash. We will ensure consistent terminology and references in future works. A comparison with RawAlign is not included, as it is based on the less efficient RawHash implementation.
RawHash2 was chosen for its superior accuracy-throughput trade-off compared to Sigmap and UNCALLED. Additionally, despite the lack of the DTW alignment step, RawHash2 introduces a highly-efficient pre-alignment search mechanism that identifies possible mappings very fast. We believe this is an important contribution that can be explored and leveraged in two different approaches: 1) for use cases that only require the mapping information and 2)  in workflows that incorporate DTW in an additional step to optimize the end-to-end pipeline. In this context, MARS accelerators can be repurposed and operate in synergy with the DTW part of such workflows e.g. SquiggleFilter.
Currently, we conduct performance comparison with tools that only do mapping, except for SquiggleFilterwhich inherently applies DTW directly to the data. We plan to revisit and improve our comparison methodology in future submissions.

\noindent
\textbf{D2. BC methodology comparison and accuracy.}
%The goal of this work is to evaluate and emulate a real-time scenario. We therefore decided to feed the same data with the same throughput to both workflows to evaluate performance. We acknowledge that basecalling is not optimized for such a setup and this is the source of the small drop in accuracy. We will explore other approaches to achieve a holistic and fair comparison. Regarding the ground truth, we have used the typical basecalling approach and used the entire genome.
The goal of this work is to evaluate and emulate a real-time scenario. 1) For performance comparison: We feed both workflows with the same data at the same throughput. The BC comparison workflow processes chunked data with a faster but less accurate basecaller, reflecting real-time constraints. We acknowledge that basecalling is not optimized for this setup, leading to a small drop in accuracy. 2) For accuracy comparison: The ground truth workflow basecalls the entire genome using a slower, more accurate basecaller, ensuring high-quality reference data.

\clearpage




==> sections/revision.tex <==
\thispagestyle{empty} % No page number
\onecolumn
\setstretch{0.9}
\noindent We thank the reviewers for their valuable feedback. We addressed reviewer concerns and improved the paper's clarity in this revision, as summarized on this page. In this document, we use \commonquestion{red for common questions}, \individualquestion{blue for individual questions}, and \minorfix{green for minor fixes}. We will further improve the paper for the next (shepherd or camera-ready) version.

{\noindent\bf\large\underline{Common Questions}}

\noindent\textbf{CQ1: Architectural Innovation (Rev B+E)} 
We acknowledge that our design is based on previous microarchitectural innovations. However, we are the first to combine these methods within an SSD, implement their orchestration, and optimize the data and control flow. Additionally, we show how our system is applied to an end-to-end application while at the same time significantly improving latency and energy consumption \textit{and} introducing algorithmic enhancements. We improved Section~\ref{sec:mech-and-sys} to highlight our innovation and make it more clear to the reader. These changes are not specific to the algorithm we base our design on. Slight modifications are possible to suit any other related algorithm that is based on the same compute primitives used in our design (i.e., arithmetic operations, filtering, sorting). This is the case for most seeding and chaining algorithms that serve as the first step in genome analysis and are therefore of high importance for this domain~\cite{alser_accelerating_2020} as other reviewers also pointed out.
%The novelty of our paper is two-fold: First, we provide the first architecture that leverages multiple different data-centric compute approaches within an SSD device for an end-to-end application. We solve the challenge of handling the data movement and communication between the different compute and storage elements and modify the algorithm such that it can be mapped to our storage-centric device. Second, we provide multiple algorithmic enhancements over the previous state-of-the-art \RSGA algorithm RawHash~\cite{firtina_rawhash_2023} that is scalable to large genomes, thereby improving the state-of-the-art accuracy results. We acknowledge that the original submission was not entirely clear about these contributions and we therefore revised section~\ref{sec:mech-overview} to address the reviewers' concerns.
\textbf{\mel{TODO}}: If enough time and space: Discussion section


\noindent\textbf{CQ2: Understanding memory usage of RSGA, roofline model (Rev A+C+D)} 

\textbf{\mel{TODO (w/ Konstantina)}}:Include roofline model + analysis section

\noindent\textbf{CQ3: General Applicability and Flexibility of the Design (Rev B+F)}
Our design implements compute patterns that are very common in the domain of genome analysis, have been used in basecalled genome analysis for several decades~\cite{alser_technology_2020}, and are now common in raw signal genome analysis~\cite{firtina_rawhash_2023}. These algorithms that use the same compute patterns could be enabled on our hardware. Additionally, seeding and chaining are essential to enable a variety of downstream tasks in the domain of genome analysis like alignment, abundance analysis or contamination analysis. Finally, several input parameters (e.g., window size and threshold for the filters, input data type, presets for seeding and chaining parameters) can be flexibly modified via software. \textbf{\mel{TODO}}: If enough time and space: Discussion section

\noindent\textbf{CQ4: Absolute evaluation values (Rev C+F)}
\textbf{\mel{TODO (w/ Rakesh)}}: Add comparison values for real time and portability analysis
\begin{itemize}
    \item Do we achieve real-time?
    \item Do we provide a portable design?
\end{itemize}


{\noindent\bf\large\underline{Individual Questions}} Labeled as: \textbf{IQ[Reviewer ID][Question Number]}, e.g., Reviewer A's first question is IQA1.

\noindent\textbf{IQA1: Blocksize of 3MB}
We increase the physical block size to minimize the space used in the internal DRAM for L2P mapping. The regular L2P is flushed to flash memory to exploit most of the internal DRAM during ISP. Any ZNS products with larger block sizes can be used on top and are therefore orthogonal to our changes.
\textbf{\mel{TODO}}: Add correct analysis of blocksize

\noindent\textbf{IQA2: Long reads of Nanopore} We fully agree with the reviewer that long reads are an important benefit of Nanopore sequencing. We already mention this benefit in Section~\ref{sec:Intro} and~\ref{sec:background} and revised our writing in Section~\ref{sec:background} to make this benefit more clear to the reader.

\noindent\textbf{IQD1: Design Choice of PNM, PUM, PNS}
Based on the initial observations we make in our motivational analysis we decide to leverage the heterogeneous storage system to tackle the I/O overhead. Within the storage system we analyze compute patterns and available compute resources (i.e., bandwidth within the SSD, already available elements, areas of accelerators we could implement) and optimize for a good trade-off between latency, area and energy. For compute patterns that take up a larger portion of the overall execution time (e.g., sorting) we design a customer accelerator so small that it makes optimal use of the internal available bandwidth. We also show why it makes sense to use the more intrusive PIM design within the internal DRAM by comparing our design (\rg) to a slightly modified design with a less complex but significanly slower PIM design of the  internal DRAM (\rgSIMDRAM). We improved our writing and explained design decisions and analysis we made in Section~\ref{sec:mech-and-sys}. Overall it would be possible to change certain design choices in order to optimize for different design points (e.g., most energy-efficient), but we decided to design a system that provides a good trade-off between all design parameters (i.e., latency, area, energy). \textbf{\mel{TODO}}: Potentially add reference to roofline model

\noindent\textbf{IQD2: Comparison to ISP}
BeaconGNN~\cite{Wang2024BeaconGNN} proposes to accelerate large-scale GNN with In-Storage Computing. The design focuses on the acceleration and evaluation of GNN which makes it hard to directly compare to our design that is targeted to end-to-end RSGA.
The introduced changes are orthogonal to our design and could be combined if required for specific applications.

ASSASIN~\cite{zou_assasin_2022} shows that the internal DRAM bandwidth can be a bottleneck for certain In Storage Processing applications. This is not the case for \proposal as we have limited data movement between the flash cells and the internal DRAM as most of the computations are performed in the internal DRAM which means we can efficiently overlap data movement and computation. Our simulator accounts for the data movement between the flash cells and the internal DRAM. The only time that we have extensive data movement during the RSGA application between DRAM and flash cells is during the sorting mechanism. However, we design our sorter such that it optimally uses the DRAM bandwidth and is not slowed down by it. Thereby we only have to introduce a sorter that is able to achieve a sorting speed matching the internal DRAM bandwidth and minimize the introduced area overhead. The proposed architecture in ASSASIN is orthogonal to our work and could be applied on top of our architecture.
We cite both paper in Section~\ref{sec:rel-work}.

Finally we also compare against a system with a conventional SSD and external accelerators added to the memory hierarchy, including ASICs and main memory DRAM-based PIM (\rgEXT). As show in Section~\ref{sec:eval-latency} it is able to improve the latency across all five datasets over the software baselines but can't match the performance and energy efficiency of our \proposal design (\rg).

\noindent\textbf{IQD3: Usage of internal DRAM}
We acknowledge that Fig. 2 might be misleading due to the visualization of the internal DRAM. We updated Fig. 2 and improved the writing such that it is clear to the reader that most of the DRAM space in conventional SSDs is used. As already mentioned by the reviewer, we put a lot of effort into shrinking the used space of the internal DRAm for our design as described in Section~\ref{sec:mech-system}.

\noindent\textbf{IQD4: Implementation details} We provide more information on the design and sizing of our sorter in Section~\ref{sec:mech-sort}. The sorter is optimized for the available internal DRAM bandwidth to provide the best trade-off between minimal latency and minimal area introduced. The sorting mechanism is not limited to the RSGA application but could also be used for other applications as it has a dedicated FSM for control.
Additionally, we added a table to summarize the SSD setup used in our simulation. It is based on a conventional SSD setup.
Moreover, we revised Section~\ref{sec:eval-accuracy} to clarify how our algorithmic modifications in \proposal improves accuracy over RawHash so much that using a fixed-point implementation can still provide better results than RawHash. However, the floating-point implementation of \proposal is better than its fixed-point implementation, as expected.

\noindent\textbf{IQE1: Comparison to other genome analysis simulators and implementations}
We'd like to clarify that all CPU centric baselines (\rhCPU, \rgCPU, \bc) are evaluated on real hardware. For our hardware implementations (\rgSIMDRAM, \rgEXT, \rg) we use a simulator for \textit{all} datasets that we evaluate. Unlike previous methods (e.g., Squigglefilter~\cite{dunn_squigglefilter_2021} that uses a costly dynamic time-warping algorithm) we use an efficient seeding algorithm that allows us to scale to larger (e.g., human) genomes. We acknowledge that it would be ideal to evaluate our proposal with real devices, however there are some challenges to do so in academia. First, even though there are some open-source SSD platforms (e.g., Cosmos+OpenSSD), the technology used for the platform is far away from modern state-of-the-art SSDs, which makes it difficult to assess the realistic impacts of ISP in modern systems.  Second, using real off-the-shelf platforms like Samsung’s SmartSSD is also problematic because it only puts an FPGA close to (but outside) a commodity SSD and packages them together. Therefore, 1) there is little flexibility to change the firmware FTL algorithm and 2) the FPGA cannot leverage the internal bandwidth of the SSD. Thus, instead of using these restrictive systems, we used simulations and HDL to model the ISP units like numerous other recent ISP works (e.g., \cite{mansouri2022genstore, mailthody2019deepstore, kim2016storage}).

\noindent\textbf{IQF1: Details on orchestration}
Once the RSGA application is initiated the SSD stops working as conventional SSD. It only performs RSGA controlled by an FSM implemented in the SSD controller. The sorter and merger are controlled by a separate FSM. No communication with the CPU is necessary during the accelerator mode and therefore no changes to the SSD-CPU interface are necessary. During accelerator mode, intermediate values are either stored in the internal DRAM or in registers near the sorters during the sorting step. Our chaining implementation uses the dynamic programming-based chaining proposed in the RawHash algorithm and is executed via the augmented computational capabilities of the internal DRAM. We improved our writing in Section~\ref{sec:mech-overview} and ~\ref{sec:mech-sort} for more clarity.

\noindent\textbf{IQF2: Comparison to basecalling baselines and alignment}
\textbf{\mel{TODO (w/ Can)}}
\begin{itemize}
    \item However, in RSGA pipelines, the alignment phase is performed using Dynamic Time Warping (DTW), which has not been optimized to the same extent as Smith-Waterman. Therefore, comparisons to prior works that adopt the BM method without including this alignment step may be unfair
\end{itemize}

\noindent\textbf{IQF3: Design Space Exploration for filters}
The final parameters used for filtering have been identified using a design space exploration. We didn't include it due to space reasons. Our design allows to flexibly chnage the parameters as input to the software, no hardware changes are needed. We modified Section~\ref{sec:mech-filt} accordingly.


\noindent\textbf{IQF4: Baseline mm2+basecaller as golden reference}
\textbf{\mel{TODO (w/ Can)}}

\noindent\textbf{IQF5: Breakdown of area and energy results}
\textbf{\mel{TODO}}

\noindent\textbf{IQF6: Scalability in Sensitivity Analysis} As stated in the text, changing the DRAM size or the number of channels by 2x is leading to a maximum speedup of 1.99x. We acknowledge that Figure 14 can be misleading and added the speedup numbers to the geomean visualization for more clarity.

\noindent\textbf{IQF7: Size of hash table} \textbf{\mel{TODO}}


==> tables/accuracy-RH-RG-only.tex <==
\begin{tabular}{@{}llrrr@{}}\toprule
\textbf{Dataset}   &           & \textbf{\rh}  & \textbf{\proposal} & \textbf{\proposal} \\
        &   &  \cite{firtina_rawhash_2023}   &   Fixed Point & Floating Point                
\\\midrule
\multicolumn{5}{c}{Read Mapping} \\\midrule
D1	            & Pr.  & 0.9868              & 0.9718  & 0.9739\\
\emph{SARS-}    & Rec.             & 0.8735              & \betterRH{0.8882} & \betterRH{0.8925}\\
\emph{CoV-2}    & $F_1$              & 0.9267         & \betterRH{0.9281} & \betterRH{0.9314}\\\midrule
D2	            & Pr.           & 0.9573           & 0.9544 & \betterRH{0.9582}\\
\emph{E. coli}  & Rec.             & 0.9009 	        & \betterRH{0.9199} & \betterRH{0.9239}\\
                & $F_1$              & 0.9282            & \betterRH{0.9368} & \betterRH{0.9408}\\\midrule
D3	            & Pr.          & \textbf{0.9862}         & 0.9417 & 0.9434\\
\emph{Yeast}    & Rec.           & 0.8412 		           & \betterRH{0.9040} & \betterRH{0.9051}\\
                & $F_1$      & 0.9079             & \betterRH{0.9225} & \betterRH{0.9239}\\\midrule
D4	            & Pr.  & 0.9691                   & 0.9084 & 0.9212\\
\emph{Green}    & Rec.     & 0.7015 		          & \betterRH{0.8120} & \betterRH{0.8361}\\
\emph{Algae}    & $F_1$     & 0.8139                  & \betterRH{0.8575} & \betterRH{0.8766}\\\midrule
D5	            & Pr.          & \textbf{0.8959}          & 0.8306 & 0.8344\\
\emph{Human}    & Rec.            & 0.4054          & \betterRH{0.4567} &  \betterRH{\textbf{0.4864}}\\
\emph{HG001}    & $F_1$         & 0.5582       & \betterRH{0.5894} &  \betterRH{\textbf{0.6146}}\\\bottomrule
\multicolumn{5}{l}{\footnotesize Pr. = Precision, Rec. = Recall} \\
\end{tabular}


==> tables/accuracy-withRH2.tex <==
\begin{tabular}{@{}llrrrrrr@{}}\toprule
\textbf{Dataset}   &           & \textbf{UNCALLED}   & \textbf{Sigmap}   & \textbf{\rh}   & \textbf{\rhtwo} & \textbf{\proposal} & \textbf{\proposal} \\
        &  &\cite{kovaka_uncalled_2021}   &  \cite{zhang_sigmap_2021}  &  \cite{firtina_rawhash_2023}  & \cite{firtina_rawhash2_2023}   &   Fixed Point & Floating Point                
\\\midrule
\multicolumn{7}{c}{Read Mapping} \\\midrule
D1	            & Pr. & 0.9547          & \textbf{0.9929} & 0.9868          & 0.9857           & 0.9718  & 0.9739\\
\emph{SARS-}    & Rec.    & \textbf{0.9910} & 0.5540          & 0.8735          & 0.8842           & \betterRH{0.8882} & \betterRH{0.8925}\\
\emph{CoV-2}    & $F_1$     & \textbf{0.9725} & 0.7112          & 0.9267          & 0.9322      & 0.9281 & 0.9314\\\midrule
D2	            & Pr. & 0.9816          & 0.9842          & 0.9573          & \textbf{0.9864}  & 0.9544 & 0.9582\\
\emph{E. coli}  & Rec.    & \textbf{0.9647} & 0.9504          & 0.9009 		 & 0.8934           & \betterRH{0.9199} & \betterRH{0.9239}\\
                & $F_1$     & \textbf{0.9731} & 0.9670          & 0.9282          & 0.9376      & 0.9368 & \betterRH{0.9408}\\\midrule
D3	            & Pr. & 0.9459          & 0.9856          & \textbf{0.9862} & 0.9567           & 0.9417 & 0.9434\\
\emph{Yeast}    & Rec.    & \textbf{0.9366} & 0.9123          & 0.8412 		 & 0.8942           & \betterRH{0.9040} & \betterRH{0.9051}\\
                & $F_1$     & 0.9412          & \textbf{0.9475} & 0.9079          & 0.9244     & 0.9225 & 0.9239\\\midrule
D4	            & Pr. & 0.8836          & \textbf{0.9741} & 0.9691          & 0.9264           & 0.9084 & 0.9212\\
\emph{Green}    & Rec.    & 0.7778          & \textbf{0.8987} & 0.7015 		 & 0.8659           & 0.8120 & 0.8361\\
\emph{Algae}    & $F_1$     & 0.8273          & \textbf{0.9349} & 0.8139          & 0.8951           & 0.8575 & 0.8766\\\midrule
D5	            & Pr. & 0.4867          & 0.4287          & \textbf{0.8959} & 0.8830           & 0.8306 & 0.8344\\
\emph{Human}    & Rec.    & 0.2379          & 0.2641          & 0.4054          & 0.4317  & \betterRH{0.4567} &  \betterRH{\textbf{0.4864}}\\
\emph{HG001}    & $F_1$     & 0.3196          & 0.3268       & 0.5582       & 0.5799  & \betterRH{0.5894} &  \betterRH{\textbf{0.6146}}\\\bottomrule
\multicolumn{5}{l}{\footnotesize Pr. = Precision, Rec. = Recall} \\
\end{tabular}


==> tables/accuracy.tex <==
\begin{tabular}{@{}llrrrrr@{}}\toprule
\textbf{Dataset}   &           & \textbf{UNCALLED}   & \textbf{Sigmap}   & \textbf{\rh}  & \textbf{\proposal} & \textbf{\proposal} \\
        &  &\cite{kovaka_uncalled_2021}   &  \cite{zhang_sigmap_2021}  &  \cite{firtina_rawhash_2023}   &   Fixed Point & Floating Point                
\\\midrule
\multicolumn{7}{c}{Read Mapping} \\\midrule
D1	            & Pr. & 0.9547          & \textbf{0.9929} & 0.9868              & 0.9718  & 0.9739\\
\emph{SARS-}    & Rec.    & \textbf{0.9910} & 0.5540          & 0.8735              & \betterRH{0.8882} & \betterRH{0.8925}\\
\emph{CoV-2}    & $F_1$     & \textbf{0.9725} & 0.7112          & 0.9267         & \betterRH{0.9281} & \betterRH{0.9314}\\\midrule
D2	            & Pr. & 0.9816          & \textbf{0.9842}          & 0.9573           & 0.9544 & \betterRH{0.9582}\\
\emph{E. coli}  & Rec.    & \textbf{0.9647} & 0.9504          & 0.9009 	        & \betterRH{0.9199} & \betterRH{0.9239}\\
                & $F_1$     & \textbf{0.9731} & 0.9670          & 0.9282            & \betterRH{0.9368} & \betterRH{0.9408}\\\midrule
D3	            & Pr. & 0.9459          & 0.9856          & \textbf{0.9862}         & 0.9417 & 0.9434\\
\emph{Yeast}    & Rec.    & \textbf{0.9366} & 0.9123          & 0.8412 		           & \betterRH{0.9040} & \betterRH{0.9051}\\
                & $F_1$     & 0.9412          & \textbf{0.9475} & 0.9079             & \betterRH{0.9225} & \betterRH{0.9239}\\\midrule
D4	            & Pr. & 0.8836          & \textbf{0.9741} & 0.9691                   & 0.9084 & 0.9212\\
\emph{Green}    & Rec.    & 0.7778          & \textbf{0.8987} & 0.7015 		          & \betterRH{0.8120} & \betterRH{0.8361}\\
\emph{Algae}    & $F_1$     & 0.8273          & \textbf{0.9349} & 0.8139                  & \betterRH{0.8575} & \betterRH{0.8766}\\\midrule
D5	            & Pr. & 0.4867          & 0.4287          & \textbf{0.8959}          & 0.8306 & 0.8344\\
\emph{Human}    & Rec.    & 0.2379          & 0.2641          & 0.4054          & \betterRH{0.4567} &  \betterRH{\textbf{0.4864}}\\
\emph{HG001}    & $F_1$     & 0.3196          & 0.3268       & 0.5582       & \betterRH{0.5894} &  \betterRH{\textbf{0.6146}}\\\bottomrule
\multicolumn{5}{l}{\footnotesize Pr. = Precision, Rec. = Recall} \\
\end{tabular}


==> tables/filters.tex <==
\begin{tabular}{@{}lrrrrr@{}}\toprule
                 & \textbf{D1} & \textbf{D2} & \textbf{D3}  & \textbf{D4} & \textbf{D5} \\\midrule
Frequency filter & 5.06\%      & 9.71\%      & 13.91\%      & 33.09\%     & 5.47\%    \\\midrule
Seed and vote    & 24.04\%     & 91.40\%     & 60.82\%      & 50.47\%     & 52.97\%    \\\midrule
Total            & 27.88\%     & 92.24\%     & 66.27\%      & 66.86\%     & 55.54\%    \\\bottomrule
% \multicolumn{7}{l}{For relative abundance estimation and contamination analysis, we combine the reads or}\\
% \multicolumn{7}{l}{reference genomes from the datasets we show in the read mapping section. We use the}\\
\end{tabular}
